A New Randomized Block-Coordinate Primal-Dual Proximal Algorithm for Distributed Optimization

This paper proposes TriPD, a new primal-dual algorithm for minimizing the sum of a Lipschitz-differentiable convex function and two possibly nonsmooth convex functions, one of which is composed with a linear mapping. We devise a randomized block-coordinate version of the algorithm which converges under the same stepsize conditions as the full algorithm. It is shown that both the original as well as the block-coordinate scheme feature linear convergence rate when the functions involved are either piecewise linear-quadratic, or when they satisfy a certain quadratic growth condition (which is weaker than strong convexity). Moreover, we apply the developed algorithms to the problem of multi-agent optimization on a graph, thus obtaining novel synchronous and asynchronous distributed methods. The proposed algorithms are fully distributed in the sense that the updates and the stepsizes of each agent only depend on local information. In fact, no prior global coordination is required. Finally, we showcase an application of our algorithm in distributed formation control.

==> TeX/Preamble/Commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% CUSTOM VARIABLES AND LENGHTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\newlength\myLength
	\newcommand\myVar{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% RENEWED COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\let\OLDhl\hl
	\renewcommand{\hl}[2][yellow]{%												highlights text (for math mode, don't use \( \) in the argument but $ $!)
		\colorlet{mycolor}{#1}%
		{\sethlcolor{mycolor}\OLDhl{#2}}%
	}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% MATH OBJECTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Symbols
	\newcommand\N{{\rm I\!N}}%													Naturals
	\newcommand\Q{\mathbb Q}%													Rationals
	\newcommand\R{{\rm I\!R}}%													Reals
	\newcommand\Rinf{\overline\R}%												Extended Reals
	\newcommand\Z{\mathbb Z}%													Integers
	\newcommand\T{{\!\intercal}}%												Transpose symbol
	
% Objects
	\newcommandx\seq[2][{2=k\in\N}]{(#1)_{#2}}%									Sequence \seq{x^k}[k\in\N]
	\newcommand\set[2]{%														Set \set{x\in\R}{x\leq a}
		\left\{
			\ifstrempty{#1}{#2}{%
				#1{}\mid{}#2%
			}%
		\right\}%
	}
	\newcommand\func[3]{#1:#2\rightarrow#3}%									f: A ---> B function \func{f}{A}{B}
	\newcommand\ffunc[3]{#1:#2\rightrightarrows#3}%								f: A ==>> B set-valued function \ffunc{f}{A}{B}
	\newcommand\innprod[2]{\left\langle#1,\:#2\right\rangle}%					Inner product
	\newcommand\tinnprod[2]{\langle#1,\:#2\rangle}%								Textstyle inner product
	\renewenvironment{cases}[1][@{}l@{}l@{}]{%									allows for additional columns in {cases}
		\left\{%
			\begin{array}{#1}
	}{%
			\end{array}
		\right.
	}
	
% Operators
	\DeclareMathOperator\ball{B}%												Ball
	\DeclareMathOperator\cl{cl}%												Set closure
	\DeclareMathOperator\conv{conv}%											Convex hull
	\DeclareMathOperator\diag{diag}%											Diagonal
	\DeclareMathOperator\dist{dist}%											Distance
	\DeclareMathOperator\dom{dom}%												Domain
	\DeclareMathOperator\epi{epi}%												Epigraph
	\DeclareMathOperator\fix{fix}%												Fixed set
	\DeclareMathOperator\gph{gph}%												Graph
	\DeclareMathOperator\im{Im}%												Image
	\DeclareMathOperator\interior{int}%											Interior
	\DeclareMathOperator\indicator{\delta}%										Indicator function
	\DeclareMathOperator\lip{lip}%												Lipschitz constant
	\DeclareMathOperator*\maximize{maximize}%									Maximize
	\DeclareMathOperator\mesh{mesh}%											Mesh of a set
	\DeclareMathOperator*\minimize{minimize}%									Minimize
	\DeclareMathOperator\proj{\Pi}%												Projection
	\DeclareMathOperator\prox{prox}%											Proximal mapping
	\DeclareMathOperator\rank{rank}%											Rank
	\DeclareMathOperator\relint{relint}%										Relative interior
	\DeclareMathOperator\sgn{sgn}%												Sign
	\DeclareMathOperator\trace{tr}%												Trace
	\DeclareMathOperator\zer{zer}%												Zeros


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% ALGORITHMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\newcommand\BREAK{\item[]{\textbf{break}}}%									\BREAK keyword
	\newcommand\algcaption[2][]{%												properly aligned algorithm caption (use in place of \caption)
		\settowidth\myLength{\textbf{Algorithm \thealgorithm~~}}%
		\caption[#1]{\begin{tabularx}{\linewidth-\myLength}[t]{@{}X@{}}#2\end{tabularx}}%
	}




==> TeX/Preamble/Local.tex <==
\newif\ifreload
\newcommand\standalone[2][width=\linewidth]{% #1=filename
	\IfFileExists{Standalone/#2.pdf}{%
		\ifreload%
			\immediate\write18{pdflatex --shell-escape --output-directory Standalone Standalone/#2.tex}%
			\immediate\write18{pdflatex --shell-escape --output-directory Standalone Standalone/#2.tex}%
			\immediate\write18{pdfannotextractor Standalone/#2.pdf}%
			\immediate\write18{pdfannotextractor Standalone/#2.pdf}%
		\fi%
	}{%
		\immediate\write18{pdflatex --shell-escape --output-directory Standalone Standalone/#2.tex}%
		\immediate\write18{pdflatex --shell-escape --output-directory Standalone Standalone/#2.tex}%
		\immediate\write18{pdfannotextractor Standalone/#2.pdf}%
		\immediate\write18{pdfannotextractor Standalone/#2.pdf}%
	}%
	\includegraphics[#1]{Standalone/#2.pdf}%
}


\definecolor{BlueIMT}{RGB}{0,42,72}

\newcommandx\file[2][{2=.tex}]{\texorpdfstring{\texttt{\small#1#2}}{#1#2}}
\newcommand\folder[1]{\texorpdfstring{\hl[cyan!15]{\texttt{\small#1/}}}{#1/}}
\newcommand\package[1]{\texorpdfstring{\hl[black!5]{\texttt{\small#1}}}{#1}}
\newcommand\command[1]{\texorpdfstring{\textcolor{green!30!black}{\textbf{\small\textbackslash#1}}}{\textbackslash#1}}

\newcommand\location[1]{%
	\hspace*{0pt}\hfill%
	\fcolorbox{cyan}{cyan!10}{%
		Commands defined in \file{TeX/Preamble/#1}%
	}%
	\vspace*{2pt}\par\noindent\ignorespaces%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  lstlisting SETTINGS  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstset{%
	backgroundcolor=\color{black!2},	% choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
	basicstyle={\tiny\ttfamily},		% the size of the fonts that are used for the code
	breakatwhitespace=false,			% sets if automatic breaks should only happen at whitespace
	breaklines=true,					% sets automatic line breaking
	captionpos=b,						% sets the caption-position to bottom
	commentstyle=\color{mygreen},		% comment style
	deletekeywords={...},				% if you want to delete keywords from the given language
	escapeinside={@(}{)@},				% if you want to add LaTeX within your code
	extendedchars=true,					% lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
%	frame=single,						% adds a frame around the code
	keepspaces=true,					% keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
	keywordstyle={\color{blue}},		% keyword style
	language=[LaTeX]tex,				% the language of the code
%	literate=*,%
  	otherkeywords={*,\\qedhere,\\cref,\\Cref,\\subsection,$,$},	% if you want to add more keywords to the set
%	numbers=left,						% where to put the line-numbers; possible values are (none, left, right)
	numbersep=5pt,						% how far the line-numbers are from the code
	numberstyle=\tiny\color{mygray},	% the style that is used for the line-numbers
%	rulecolor=\color{black},			% if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
	showspaces=false,					% show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
	showstringspaces=false,				% underline spaces within strings only
	showtabs=false,						% show tabs within strings adding particular underscores
	stringstyle=\color{mymauve},		% string literal style
	tabsize=2,							% sets default tabsize to 2 spaces
%	title=\lstname,						% show the filename of files included with \lstinputlisting; also try caption instead of title
}



==> TeX/Preamble/Packages.tex <==
\usepackage[noend]{algorithmic}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage[margin=1em]{caption}
\usepackage{comment}%															For \begin{comment} --- \end{comment} comments
\usepackage[english]{babel}%													English hyphenation
%
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[babel]{csquotes}%													Load after inputenc
\usepackage{multirow}%															For table cells spanning multiple rows
\usepackage{nicefrac}%															1-liner fractions with \nicefrac
\usepackage{refcount}%															\getrefcounter{label} to get value of counter labelled with label
\usepackage{soulutf8}%															Needed for \hl command (highlighting text)
\usepackage{tabularx}%															For fullwidth justified columns (X)
\usepackage{xpatch}
\usepackage[%
	abbr,
	appendix,
	extras,
]{clevethm}
\usepackage{tikz}
	\usetikzlibrary{arrows}
	\usetikzlibrary{calc}
	\usetikzlibrary{decorations.markings}
	\usetikzlibrary{positioning}
	\usetikzlibrary{through}
%	\usetikzlibrary{external}
%\tikzsetexternalprefix{Pics/Tikz/}
%\tikzexternalize
\usepackage{pgfplots}
	\usepgfplotslibrary{fillbetween}
%	\tikzexternalize
	\pgfplotsset{compat=1.10}
\usepackage{algorithm}
%  \usepackage[noend]{algpseudocode}
%\usepackage[compatible]{algpseudocode} 
 %or
%  \usepackage{algcompatible}

\usepackage[normalem]{ulem}



==> TeX/Preamble/additional_Commands.tex <==
%\usepackage{mathbbol}  % for mathbb of digits changes regular one though
%\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx

%\usepackage{dsfont} % for mathbb of numbers 

\newcommand\mathtight{%														% Tightens math equation
	\thinmuskip=1mu%	Unary operator-arg	sin·x   Default: 3mu
	\medmuskip=2mu%		Binary operator-LR	x·+·y   Default: 4mu
	\thickmuskip=4mu%	Relations-LR		x·=·y   Default: 5mu plus 5mu
	\renewcommand\quad{\hspace*{0.5em}}
	\renewcommand\qquad{\quad\quad}
}%

%\usetikzlibrary{pgfplots.groupplots,matrix}
%\usetikzlibrary{external}


% commands 
\newcommand{\bld}[1]{\boldsymbol{#1}}

\newcommand{\lb}[1]{ {\underline {#1}}} %lower bounds
\newcommand{\ub}[1]{ {\overline {#1}}} %upper bounds
\newcommand{\stsum}[1]{\displaystyle\sum\limits #1} % nice sum
\newcommand{\pte}[1]{ ~\mbox{\color{red} #1}} % pano's comments in equations
\newcommand{\pt}[1]{{\color{red} #1}} % pano's comments
\newcommand{\smallmat}[1]{\left[ \begin{smallmatrix}#1 \end{smallmatrix} \right]}
\newcommand{\eqdef}{\triangleq}
\newcommand{\cprod}{\ell_{\mathrm{prod}}}


\newcommand{\ri}{\mathop{\rm ri}\nolimits}

\newcommand{\cone}{\mathop{\rm cone}\nolimits}
\newcommand{\rint}{\mathop{\rm rint}\nolimits}
\newcommand{\lev}{\mathop{\rm lev}\nolimits}
\newcommand{\aff}{\mathop{\rm aff}\nolimits}
\newcommand{\supp}{\mathop{\rm supp}\nolimits}
\newcommand{\Int}{\mathop{\rm int}\nolimits}
\newcommand{\id}{\mathop{\rm Id}\nolimits}


\newcommand{\blkdiag}{\mathop{\rm blkdiag}\nolimits}
\newcommand{\df}{\mathrm{d}f}
\newcommand{\ddf}{\mathrm{d}^2f}


\newcommand{\ddiag}{\mathop{\rm diag}\nolimits}
\newcommand{\sign}{\mathop{\rm sign}\nolimits}
\newcommand{\soft}{\mathop{\rm soft}\nolimits}
\newcommand{\lmigeq}{\succcurlyeq}


% Sets
\renewcommand{\Re}{{\rm{I\!R}} }

\newcommand{\Nn}{{\rm{I\!N}}}
\newcommand{\Bb}{{\rm I\!B} }
% Hilbert spaces
\newcommand{\ZZ}{\mathcal Z}
\newcommand{\HH}{\mathcal H}
\newcommand{\GG}{\mathcal G}
\newcommand{\KK}{\mathcal K}
\newcommand{\YY}{\mathcal Y}
\newcommand{\XX}{\mathcal X}
% set-valued mappings
\newcommand{\rra}{\rightrightarrows}


\newcommand{\sol}{\mathop{\rm SOL}\nolimits}

\newcommand{\gra}{\mathop{\rm gra}\nolimits}

%\newcommand{\argmin}{\mathop{\rm arg\ min}\nolimits}
%\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmin}{\arg\!\min}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\stt}{\rm subject\ to}

\newcommand{\ie}{\emph{i.e.}}

\DeclareMathOperator*{\E}{\mathbb{E}}

%\newcommand{\onebb}{{\sf 1\hspace{-2.5pt}I}}
%\newcommand{\onebb}{{\rm 1\hspace{-3.5pt}1}}
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}

%\newcommand{\bld}[1]{\boldsymbol{#1}}

\tikzstyle{every picture}+=[remember picture]
\tikzstyle{na} = [baseline=-.5ex]
\tikzstyle{every picture}+=[remember picture]
\tikzstyle{na} = [baseline=-.5ex]


\newcommand\Rect[1]{	\tikz[baseline=(char.base)]\node[rectangle,draw , cyan,rounded corners,inner sep=2pt] (char) {#1};}

\newcommand\Rectr[1]{	\tikz[baseline=(char.base)]\node[rectangle,draw , black!30!orange,rounded corners,inner sep=2pt] (char) {#1};}

\newcommand\Rectg[1]{	\tikz[baseline=(char.base)]\node[rectangle,draw , black!30!green,rounded corners,inner sep=2pt] (char) {#1};}



% this is necessary for using background enviroment of pgfplot
\pgfdeclarelayer{background}
\pgfsetlayers{background,main}

%Nick's
%\newcommand{\N}{\mathcal{N}}
\newcommand{\Ne}{\mathcal{N}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Nin}{\mathcal{N}^{\text{in}}}
\newcommand{\Nout}{\mathcal{N}^{\text{out}}}

\newcommand{\x}{\mathsf{x}}
\newcommand{\y}{\mathsf{y}}
\newcommand{\w}{\mathsf{w}}

\newcommand{\f}{\mathsf{f}}
\newcommand{\g}{\mathsf{g}}
\newcommand{\h}{\mathsf{h}}



%\renewcommand{\S}{\mathcal{S}}
\newcommand{\F}{\mathcal{F}}

\newcommand{\hide}[1]{}
%\newcommand{\done}{\centerline{\textbf{\color{blue} **DONE UP TO HERE**}}}
\definecolor{mygreen}{rgb}{0.0, 0.5, 0.0}
\def\nf#1{{\color{red}#1}}
%\def\nf#1{#1}
\def\nfc#1{\textbf{{\color{purple}NF: #1}}}

\newcommand{\done}{\centerline{\textbf{\color{mygreen} **NF: EDITED UP TO HERE**}}}

\def\pp#1{{\color{red}#1}}




==> TeX/Text/Algorithm.tex <==
 Consider the following algorithm that is based on \cite[Algorithm 3]{AFBA2016} with change or order and when $\mu=0$ and $\alpha_n=1$: 
 \begin{align*}
 \bar{y}_{k}&=\prox_{\gamma_{2}h^{\star}}(y_{k}+\gamma_{2}Lx_{k})\\\bar{x}_{k}&=\prox_{\gamma_{1}g}(x_{k}-\gamma_{1}\nabla f(x_{k})-\gamma_{1}L^{*}(\theta\bar{y}_{k}+(1-\theta)y_{k}))\\x_{k+1}&=\bar{x}_{k}\\y_{k+1}&=\bar{y}_{k}+\gamma_{2}(2-\theta)L\tilde{x}_{k}.
 \end{align*}
 This is the case where $$S=\left[\begin{array}{cc}
 \gamma_{2}^{-1} & -(1-\theta)L\\
 -(1-\theta)L^{*} & \gamma_{1}^{-1}+(1-\theta)(2-\theta)\gamma_{2}L^{*}L
 \end{array}\right],$$
 and 
 \begin{equation} \label{eq:PD}
P=\left[\begin{array}{cc}
\gamma_{2}^{-1} & \frac{\theta}{2}L\\
\frac{\theta}{2}L^{*} & \gamma_{1}^{-1}
\end{array}\right], \quad 
D=\left[\begin{array}{cc}
\gamma_{2}^{-1} & L\\
L^{*} & \gamma_{1}^{-1}+\gamma_{2}(2-\theta)L^{*}L
\end{array}\right] 
 \end{equation} 
 
 Let us define a new set of variables $\bar{z}_k^n=(\bar{x}_k^n,\bar{y}_k^n)=(\bar{x}_k,\bar{y}_k+\gamma_2(2-\theta)L(\bar{x}_k-x_k))$. 
 The asynchronous algorithm is then defined as follows: 
 
  \begin{align*}
  \bar{y}_{k}&=\prox_{\gamma_{2}h^{\star}}(y_{k}+\gamma_{2}Lx_{k})\\\bar{x}_{k}&=\prox_{\gamma_{1}g}(x_{k}-\gamma_{1}\nabla f(x_{k})-\gamma_{1}L^{*}(\theta\bar{y}_{k}+(1-\theta)y_{k}))\\\bar{z}_k^n=&(\bar{x}_k,\bar{y}_k+\gamma_2(2-\theta)L(\bar{x}_k-x_k))\\
  z_{k+1}=& z_k + U_{i_k}(\bar{z}_k^n-z_k). 
  \end{align*}
  where $U_iz=(0,\ldots,z_i,0,\ldots,0)$. For simplicity we'll assume the $i_k$ is an i.i.d sequence with a uniform probability distribution (This can probably be relaxed). We denote by $\mathcal{F}_k$ the filteration generated by the random variable $i_k$ and will write $\mathbb{E}_k\left[\cdot\right]$ in place of $\mathbb{E}_k\left[\cdot|\mathcal{F}_k\right]$ for notation simplicity.   
  \begin{lem} \label{lem:Fejerlike}
  	Let $z_{n}$ be the sequence generated by our scheme. For every $\mathcal{F}_k$  measurable  random variable $Z$ we have
  	\footnotesize\begin{align}
  	{\mathbb{E}_k}\left[\|z_{k+1}-Z\|_{S}^{2}\right]	
  	\leq (1-\frac{1}{m})\|z_{k}-Z\|_{S}^{2}+\frac{1}{m}\|\bar{z}^n_{k}-Z\|_{S}^{2}+\frac{\|S\|\|S^{-1}\|-1}{m}\|\bar{z}^n_k-{z}_{k}\|_{S}^{2}. \label{eq:Fejerlike}
  	\end{align} \normalsize
  	  	In particular, we have 
\begin{equation}\label{eq:-8}
	{\mathbb{E}_k}\left[\|z_{k+1}-z_k\|_{S}^{2}\right]	
	\leq \frac{\|S\|\|S^{-1}\|}{m}\|\bar{z}^n_k-{z}_{k}\|_{S}^{2}.
\end{equation}
  	\end{lem}  
  	\begin{proof}
  			 We have 
  			 \footnotesize
  			 \begin{align}
  			 {\mathbb{E}_k}\left[\|z_{k+1}-Z\|_{S}^{2}\right]	&=	{\mathbb{E}}\left[\|z_{k}-Z+U_{i_{k}}(\bar{z}^n_k-z_k)\|_{S}^{2}\right]\nonumber\\
  			 &=	\|z_{k}-Z\|_{S}^{2}+{\mathbb{E}_k}\left[2\langle z_{k}-Z,U_{i_{k}}(\bar{z}^n_k-z_k)\rangle_{S}+\|U_{i_{k}}(\bar{z}^n_k-z_k)\|_{S}^{2}\right]\nonumber\\
  			 &=	\|z_{k}-Z\|_{S}^{2}-\sum_{i=1}^{m}\frac{2}{m}\langle z_{k}-Z,U_{i_{k}}(\bar{z}^n_k-z_k)\rangle_{S}+\sum_{i=1}^{m}\frac{1}{m}\|U_{i_{k}}(\bar{z}^n_k-z_k)\|_{S}^{2}. \label{eq:-1}
  			 \end{align} \normalsize
  			 
  			 
  			  For the inner product in the right hand side above we have 
  			  \begin{align}
  			  \sum_{i=1}^{m}\langle z_{k}-Z,U_{i_{k}}(\bar{z}^n_k-z_k)\rangle_{S}	&=	\sum_{i=1}^{m}\langle Sz_{k}-SZ,U_{i_{k}}(\bar{z}^n_k-z_k)\rangle\nonumber\\&=\langle Sz_{k}-SZ,\bar{z}^n_k-z_k\rangle  =\langle z_{k}-Z,\bar{z}^n_k-z_k\rangle_S
  			  \label{eq:-3}\end{align}
  			  For the last term in~\eqref{eq:-1} we have 
  			  \begin{align}
  			  \sum_{i=1}^{m}\|U_{i_{k}}(\bar{z}^n_k-z_k)\|_{S}^{2}& \leq \sum_{i=1}^{m}\|S\|\|U_{i_{k}}(\bar{z}^n_k-z_k)\|^{2}= \|S\|\|\bar{z}^n_k-z_k\|^{2}\nonumber\\
  			  &\leq \|S\|\|S^{-1}\|\|\bar{z}^n_k-z_k\|_{S}^{2}. \label{eq:-2}
  			  \end{align}	
  			  Combining~\eqref{eq:-1},~\eqref{eq:-3} and~\eqref{eq:-2} yields 
  			  \footnotesize
  			  	 \begin{align*}
  			  	 {\mathbb{E}_k}\left[\|z_{k+1}-Z\|_{S}^{2}\right]	&=	\|z_{k}-Z\|_{S}^{2}-\sum_{i=1}^{m}\frac{2}{m}\langle z_{k}-Z,U_{i_{k}}(\bar{z}^n_k-z_k)\rangle_{S}+\sum_{i=1}^{m}\frac{1}{m}\|U_{i_{k}}(\bar{z}^n_k-z_k)\|_{S}^{2}\\
  			  	 &\leq \|z_{k}-Z\|_{S}^{2}+ \frac{2}{m}\langle z_{k}-Z,\bar{z}^n_k-z_k\rangle_S + \frac{\|S\|\|S^{-1}\|}{m} \|\bar{z}^n_k-z_k\|_{S}^{2} \\
  			  	 &= (1-\frac{1}{m})\|z_{k}-Z\|_{S}^{2}+\frac{1}{m}\|\bar{z}^n_{k}-Z\|_{S}^{2}+\frac{\|S\|\|S^{-1}\|-1}{m}\|\bar{z}^n_k-{z}_{k}\|_{S}^{2},
  			  	 \end{align*} \normalsize
  			  where we used the identity $2\langle a,b\rangle_S=\|a+b\|^2_S-\|a\|^2_S-\|b\|^2_S$ in the last equality. 
  		\end{proof}
  		In \Cref{lem:Fejerlike} the main difference with \cite[Lemma 2]{fercoq2015coordinate} is that when $L$ has only one nonzero element at each row and $P$ has scalar diagonals then the last term in~\eqref{eq:Fejerlike} disappears. 
  		\begin{lem}\label{lem:nablaf}
  			Let $P,D$ be defined as in \cite{AFBA2016}. Assume $c P \succeq D$ (this implies $c>1$). Then we have
  			\begin{equation*}
  			\langle\nabla f(x^{\star})-\nabla f(x_{k}),x^{\star}-\bar{x}^n_{k}\rangle+(c^{-1}-\frac{1}{2})\|\bar{z}_{k}^{n}-z_{k}\|_{S}^{2}\leq-\frac{1}{2}\|\bar{z}_{k}^{n}-z^{\star}\|_{S}^{2}+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}
  			\end{equation*}
  			\end{lem}
  			\begin{proof}
  				Following the reasoning in the proof of \cite[Theorem 3.1]{AFBA2016} we have: 
  				\begin{equation}
  				\langle\nabla f(x^{\star})-\nabla f(x_{k}),x^{\star}-\bar{x}\rangle+\|\tilde{z}_{k}\|_{P}^{2}\leq\langle z_{k}-z^{\star},-(M^{*}+H)\tilde{z}_{k}\rangle.
  				\end{equation}\label{eq:-5}
  				We saw that $S^{-1}(H+M^*)\tilde{z}_k=\bar{z}_k^n-z_k$. Thus
  				\begin{align}
  				\langle z_{k}-z^{\star},-(M^{*}+H)\tilde{z}_{k}\rangle &= \langle z_{k}-z^{\star},-\bar{z}_{k}^{n}+z_{k}\rangle_S \nonumber\\ & = -\frac{1}{2}\|\bar{z}_{k}^{n}-z^{\star}\|_{S}^{2}+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}+\frac{1}{2}\|\bar{z}_{k}^{n}-z_{k}\|_{S}^{2}.\label{eq:-6}
  				\end{align}
  				Furthermore we have 
  				\begin{equation}\label{eq:-7}
  				\|\tilde{z}_{k}\|_{P}^{2}\geq c^{-1}\|\tilde{z}_{n}\|_{D}^{2}=c^{-1}\|S^{-1}(H+M^{*})\tilde{z}_{n}\|_{S}^{2}=c^{-1}\|\bar{z}_{k}^{n}-z_{k}\|_{S}^{2}.
  				\end{equation}
  				Combining~\eqref{eq:-5}, \eqref{eq:-6} and~\eqref{eq:-7} completes the proof. 
  				\end{proof}
  				
  				\begin{rem}
  					Consider the condition $c P\succeq D$ for $P$ and $D$ defined in~\eqref{eq:PD}. Using Schur complement yields the following sufficient condition:
  					\begin{equation} \label{eq:c}
  					(c-1)^2 - \gamma_1\gamma_2\|L\|^2\left((2-\theta)(c-1)+(\frac{c\theta}{2}-1)^2\right)\geq 0
  					\end{equation}
  				\end{rem}
  				
				\begin{lem}\label{lem:main}
				\textcolor{red}{Let our assumptions hold}. Define
				\begin{equation}\label{eq:S}
				S_k^\star = f(x_k)-f(x^\star) - \langle\nabla f(x^\star),x_k-x^\star\rangle.
				\end{equation}	
				Then the following inequality holds: 
				\small
				\begin{align*}
				\mathbb{E}_{k}\left[ S_{k+1}^\star+\frac{1}{2}\left[\|z_{k+1}-z^{\star}\|_{S}^{2}\right]\right]\leq  
				(1-\frac{1}{m})S_k^\star-\frac{1}{m}\tilde{V}(\bar{z}^n_{k}-z_k)+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}.
				\end{align*}\normalsize
				where $\tilde{V}(z)=\left(\frac{c^{-1}}{\|S\|\|S^{-1}\|}-\frac{1}{2}\right)\|z\|_{S}^{2}-\frac{1}{2}\|x\|_\beta^{2}$ and $\beta=(\beta_1,\cdots,\beta_m)$. 
					\end{lem}
					\begin{proof}
						It follows from \Cref{lem:Fejerlike} at point $z^\star$ that: 
						  	\begin{align*}
						  	{\mathbb{E}_k}\left[\|z_{k+1}-z^\star\|_{S}^{2}\right]	
						  	\leq (1-\frac{1}{m})\|z_{k}-z^\star\|_{S}^{2}+\frac{1}{m}\|\bar{z}^n_{k}-z^\star\|_{S}^{2}+\frac{\|S\|\|S^{-1}\|-1}{m}\|\bar{z}^n_k-{z}_{k}\|_{S}^{2}.
						  	\end{align*}
						  	Using this together with~\Cref{lem:nablaf} yields
						  		\begin{equation*}
						  		\langle\nabla f(x^{\star})-\nabla f(x_{k}),x^{\star}-\bar{x}_{k}^{n}\rangle+\left(c^{-1}-\frac{\|S\|\|S^{-1}\|}{2}\right)\|\bar{z}_{k}^{n}-z_{k}\|_{S}^{2}\leq-\frac{m}{2}{\mathbb{E}_{k}}\left[\|z_{k+1}-z^{\star}\|_{S}^{2}\right]+\frac{m}{2}\|z_{k}-z^{\star}\|_{S}^{2}
						  		\end{equation*}
						  	Next we divide both sides by $m$ and use $\mathbb{E}_{k}[x_{k+1}]=\frac{1}{m}\bar{x}_{k}^{n}+(1-\frac{1}{m})x_{k}$  to derive: 
							\small
						  	\begin{align*}\langle\nabla f(x^{\star})-\nabla f(x_{k}),-\mathbb{E}_{k}[x_{k+1}]+x_{k}\rangle+\frac{1}{m}\left(c^{-1}-\frac{\|S\|\|S^{-1}\|}{2}\right)\|\bar{z}_{k}^{n}-z_{k}\|_{S}^{2}\leq & \\
						  	\frac{1}{m}\langle\nabla f(x^{\star})-\nabla f(x_{k}),x_{k}-x^{\star}\rangle-\frac{1}{2}{\mathbb{E}_{k}}\left[\|z_{k+1}-z^{\star}\|_{S}^{2}\right]+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}
						  	\end{align*}
						  	\normalsize
						  %	Use~\eqref{eq:-8} to derive						 	\begin{align*}\langle\nabla f(x^{\star})-\nabla f(x_{k}),-\mathbb{E}_{k}[x_{k+1}]+x_{k}\rangle+\left(\frac{c^{-1}}{\|S\|\|S^{-1}\|}-\frac{1}{2}\right){\mathbb{E}_k}\left[\|z_{k+1}-z_k\|_{S}^{2}\right]\leq & \\						  	\frac{1}{m}\langle\nabla f(x^{\star})-\nabla f(x_{k}),x_{k}-x^{\star}\rangle-\frac{1}{2}{\mathbb{E}_{k}}\left[\|z_{k+1}-z^{\star}\|_{S}^{2}\right]+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}.						  	\end{align*}
						Equivalently
						\begin{align*}
						\mathbb{E}_{k}\left[\langle\nabla f(x^{\star})-\nabla f(x_{k}),-x_{k+1}+x_{k}\rangle\right]+\frac{1}{m}\left(c^{-1}-\frac{\|S\|\|S^{-1}\|}{2}\right)\|\bar{z}_{k}^{n}-z_{k}\|_{S}^{2}\leq & \\
						\frac{1}{m}\langle\nabla f(x^{\star})-\nabla f(x_{k}),x_{k}-x^{\star}\rangle-\frac{1}{2}{\mathbb{E}_{k}}\left[\|z_{k+1}-z^{\star}\|_{S}^{2}\right]+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}.
						\end{align*}
						Next we use coordinate wise Lipschitz knowing that $x_{k+1}$
						differs from $x_{k}$
						along coordinate $i_{k+1}$	only: 
						\begin{equation}
						f(x_{k+1})\leq f(x_{k})+\langle\nabla f(x_{k}),x_{k+1}-x_{k}\rangle+\frac{\beta_{i_{k+1}}}{2}\|x_{k+1}-x_{k}\|^{2}
						\end{equation}
						Using this we derive 
						\footnotesize
							\begin{align*}
							\mathbb{E}_{k}\left[f(x_{k+1})-f(x_{k})-\frac{\beta_{i_{k+1}}}{2}\|x_{k+1}-x_{k}\|^{2}-\langle\nabla f(x^{\star}),x_{k+1}-x_{k}\rangle\right]+\frac{1}{m}\left(c^{-1}-\frac{\|S\|\|S^{-1}\|}{2}\right)\|\bar{z}_{k}^{n}-z_{k}\|_{S}^{2}\leq & \\
							\frac{1}{m}\langle\nabla f(x^{\star})-\nabla f(x_{k}),x_{k}-x^{\star}\rangle-\frac{1}{2}{\mathbb{E}_{k}}\left[\|z_{k+1}-z^{\star}\|_{S}^{2}\right]+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}.
							\end{align*}
						\normalsize 
						From convexity of $f$, we have  $$\langle\nabla f(x^{\star})-\nabla f(x_{k}),x_{k}-x^{\star}\rangle\leq\langle\nabla f(x^{\star}),x_{k}-x^{\star}\rangle+f(x^{\star})-f(x_{k})=-S_{k}^{*}.$$ This together with definition of $S_k^\star$ yields
						\footnotesize
						\begin{align*}
						\mathbb{E}_{k}\left[ S_{k+1}^\star-\frac{\beta_{i_{k+1}}}{2}\|x_{k+1}-x_{k}\|^{2}\right]+\frac{1}{m}\left(c^{-1}-\frac{\|S\|\|S^{-1}\|}{2}\right)\|\bar{z}_{k}^{n}-z_{k}\|_{S}^{2}\leq %& \\
						(1-\frac{1}{m})S_k^\star-\frac{1}{2}{\mathbb{E}_{k}}\left[\|z_{k+1}-z^{\star}\|_{S}^{2}\right]+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}.
						\end{align*}
						\normalsize 
						Next we note that $\mathbb{E}_k\left[\|x_{k+1}-x_k\|^2\right]= \sum_{i=1}^{m}\frac{1}{m}\|(\bar{x}^n_{k})^i-x_k^i\|= \frac{1}{m}\|\bar{x}^n_{k}-x_k\|^2$. Using this and rearranging yields the result. 						
						\end{proof}
  			
  			
  			\section{Special case: $\theta=1$}
  			
			In this special case the algorithm becomes: 
			  \begin{align*}
			  \bar{y}_{k}&=\prox_{\gamma_{2}h^{\star}}(y_{k}+\gamma_{2}Lx_{k})\\\bar{x}_{k}&=\prox_{\gamma_{1}g}(x_{k}-\gamma_{1}\nabla f(x_{k})-\gamma_{1}L^{*}\bar{y}_{k})\\\bar{z}_k^n=&(\bar{x}_k,\bar{y}_k+\gamma_2L(\bar{x}_k-x_k))\\
			  z_{k+1}=& z_k + U_{i_k}(\bar{z}_k^n-z_k). 
			  \end{align*}
		
			 This is the case where $$S=\diag(\gamma_2^{-1},\gamma_1^{-1}),$$
			 and 
			 \begin{equation} \label{eq:PD}
			 P=\left[\begin{array}{cc}
			 \gamma_{2}^{-1} & \frac{1}{2}L\\
			 \frac{1}{2}L^{*} & \gamma_{1}^{-1}
			 \end{array}\right], \quad 
			 D=\left[\begin{array}{cc}
			 \gamma_{2}^{-1} & L\\
			 L^{*} & \gamma_{1}^{-1}+\gamma_{2}L^{*}L
			 \end{array}\right] 
			 \end{equation} 

\begin{ass} 
	\begin{enumerate}
		\item Let 
		\begin{equation}
		\sum_{i=1}^{m} U_i = \id.
		\end{equation}
		\item $\gamma^{i}_1 < \frac{2c^{-1}-1}{\beta_i}$
	\end{enumerate}
	\end{ass}
	

	
	  \begin{lem} \label{lem:Fejerlike-t1}
	  	Let $z_{n}$ be the sequence generated by our scheme. For every $\mathcal{F}_k$  measurable  random variable $Z$ we have
	  	\footnotesize\begin{align}
	  	{\mathbb{E}_k}\left[\|z_{k+1}-Z\|_{S}^{2}\right]	
	  	= (1-\frac{1}{m})\|z_{k}-Z\|_{S}^{2}+\frac{1}{m}\|\bar{z}^n_{k}-Z\|_{S}^{2}. \label{eq:Fejerlike-t1}
	  	\end{align} \normalsize
	  	In particular, we have 
	  	\begin{equation}\label{eq:-8-t1}
	  	{\mathbb{E}_k}\left[\|z_{k+1}-z_k\|_{S}^{2}\right]	
	  	\leq \frac{1}{m}\|\bar{z}^n_k-{z}_{k}\|_{S}^{2}.
	  	\end{equation}
	  \end{lem}  
	  
	\begin{proof}
		 The proof is identical to the proof of \Cref{lem:Fejerlike} but in this case we have
			  \begin{align}
			  \sum_{i=1}^{m}\|U_{i_{k}}(\bar{z}^n_k-z_k)\|_{S}^{2} = \sum_{i=1}^{m}\gamma_i\|U_{i_{k}}(\bar{z}^n_k-z_k)\|^{2}= \|\bar{z}^n_k-z_k\|_{S}^{2}. \label{eq:-2-t1}
			  \end{align}	
		\end{proof}
		
		\Cref{lem:nablaf} remains valid but \Cref{lem:main} is relaxed to the following 
		\begin{lem}\label{lem:main-t1}
			\textcolor{red}{Let our assumptions hold}. Define
			\begin{equation}\label{eq:S}
			S_k^\star = f(x_k)-f(x^\star) - \langle\nabla f(x^\star),x_k-x^\star\rangle.
			\end{equation}	
			Then the following inequality holds: 
			\small
			\begin{align*}
			\mathbb{E}_{k}\left[ S_{k+1}^\star+\frac{1}{2}\left[\|z_{k+1}-z^{\star}\|_{S}^{2}\right]\right]\leq  
			(1-\frac{1}{m})S_k^\star-\frac{1}{m}\tilde{V}(\bar{z}^n_{k}-z_k)+\frac{1}{2}\|z_{k}-z^{\star}\|_{S}^{2}.
			\end{align*}\normalsize
			where $\tilde{V}(z)=\left({c^{-1}}-\frac{1}{2}\right)\|z\|_{S}^{2}-\frac{1}{2}\|x\|_\beta^{2}$ and $\beta=(\beta_1,\cdots,\beta_m)$. 
		\end{lem}
		
		The condition~\eqref{eq:c} in this case simplifies to $c= \frac{1}{1-\sqrt{\gamma_1\gamma_2\|L\|^2}/2}$. Thus we get 
		
		$\gamma_1^i \beta_i < 1 - \sqrt{\gamma_1\gamma_2 \|L\|^2}$.
		\textcolor{red}{Write everything properly, it seems to work perfectly!} 
		
		

		
		Consider the following problem 
		
			\begin{subequations} \label{prob:GenProblem}
				\begin{align}
				\minimize&\quad \sum_{i=1}^Nf_i(x_i)+g_i(x_i)+h_i\left(L_ix_i\right)\\\stt&\quad A_{ij}x_i + A_{ji}x_j=b_{(i,j)}
				\qquad(i,j)\in E%\; (\forall j\in{\mathcal{N}_i}) \qquad\textrm{for} \;i=1,\cdots,M \;
				\end{align}
			\end{subequations}
		
		

==> TeX/Text/NUM.tex <==
%!TEX root = ../../paper.tex

\textcolor{blue}{Can we have a quadratic term?}

In this section, we showcase an application of our distributed algorithm to \emph{Network Utility Maximization} (NUM), a popular framework used for resource allocation in multi-commodity networks, with applications ranging from wireline and wireless communication networks~\cite{srikant2013communication}, to industrial assembly lines and smart transportation systems. 
%
For illustration, we 
%
%wireline and wireless networks~\cite{srikant2013communication}. 
%~\cite{lin2004joint,tassiulas1992stability}. 
%In the following, we treat a general case of NUM for \emph{wireless networks} which results to the celebrated cross-layer design %~\cite{lin2006tutorial}, \ie, the coupling of the transport layer, the network layer and the data link layer for jointly dynamically performing congestion control, routing and Medium Access Control (MAC) in wireless networks.  We note in passing that this formulation may capture various applications pertinent to resource allocation networks with conflict constraints and multi-commodity flows, with a notable recent example being traffic control in transportation networks.%~\cite{gregoire2015capacity}. 
%We 
assume a wireless communication network %consisting of $N$ nodes (enumerated as $1,2,\hdots,N$), 
with topology captured by an undirected %\footnote{For simplicity, communication is taken symmetric, e.g., all nodes are assumed to utilize the same transmission power.} 
graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where node $i$ can transmit data to node $j$ if and only if $(i,j)\in \mathcal{E}$.  For a node $i\in\mathcal{V}$ we define its 
neighborhood $\Ne_i:=\{j \mid (i,j) \in \mathcal{E}\}$.
%in-neighborhood $\Nin_i := \{j| (j,i) \in E\}$, and its out-neighborhood $\Nout_i := \{j| (i,j) \in E\}$. We also let $M:=\|E\|$ the number of links.

Let $\F\subseteq \mathcal{V} \times \mathcal{V}$ be a set of source-destination pairs, alternatively called \emph{users}, which correspond to end-to-end traffic flows in the network. For simplicity, we allow for 
two users to share a common source node or destination node, but not both.
% 
%
We denote by $\mathcal{S}\subseteq\mathcal{V}$ and $\D\subseteq\mathcal{V}$ the set of source and destination nodes respectively. For every $i\in\mathcal{S}$, $\D_i$ denotes the set of nodes $d\in\mathcal{D}$ for which $(i,d)\in\mathcal{F}$, \emph{i.e.}, the set of destination nodes whose source is node $i$. If $i\notin \mathcal{S}$,  \emph{i.e.}, if $i$ is not the source of any user, then we define $\mathcal{D}_i = \varnothing $. For $i\in\mathcal{V}$, we denote by $\D_{-i}:=\D \setminus\{\D_i\cup \{i\}\}$ the set of destination nodes different than $i$  with a source other than $i$. 
%
%
For each $i\in\mathcal{S}$, $d\in \D_i$, we use $x^d_i$ to denote the \emph{flow rate} for user $(i, d)\in\mathcal{F}$.  
%Last, for $i\in\mathcal{V}$, we denote by \nf{$\D_{-i}:=\D \setminus\{i\}$} the set of destination nodes different than $i$ (by definition, $\D_{-i}=\D$, for $i\notin\D$).

%enumerated as $1,2,\hdots,F$. 
%For each user $f\in\F$ we let $s_f,d_f \in \mathcal{V}$ denote the \nf{corresponding} source and destination nodes, respectively. We let 
%%$\{x_{s}\}_{s\in S}$ denote their  (average) rates. Let 
%$x_f$ denote the \emph{flow rate} (a decision variable corresponding to flow control of exogenous traffic into the network). %, and $s_f,d_f$ denote the source and destination nodes, respectively. 
%\nf{Additionally, we define the set $\D$ of destinations, i.e., the set of nodes such that there exists at least one user designating traffic towards them, $\D=\cup_{i\in \mathcal{V}_s}\{\D_i\}\subseteq \mathcal{V}$.}

For each $(i,j)\in \mathcal{E}$, we call the directed pair $ij$ the \emph{link} with node $i$ being the transmitter and node $j$ the receiver. We define link rates, \emph{separately for each destination}\footnote{Note that two different users may have the same destination 
(but different source). It is customary to maintain, for each link, a single \emph{queue} for the cumulative traffic towards 
a given destination, which justifies the convention for per-destination rates  $\{r_{ij}^d\}$.}~\cite{srikant2013communication} as follows:  %\footnote{We may alternatively consider per user link rates, but it is customary to consider per destination queues in packet networks, hence the link rates are defined for each destination node. Note that several users may share a common source or destination, however traffic is handled in a per destination fashion~\cite{srikant2013communication}.}. 
  for $(i,j)\in \mathcal{E}$, let $r^d_{ij}$ be the transmission rate from node $i$ to node $j$, cumulative over all flows with common destination $d$; these are decision variables related to scheduling (MAC) as well as dynamic routing (when user routes are not determined beforehand). The total link rate (over all flows) is given by $r_{ij} := \sum_d r_{ij}^d$; without any loss of generality, we adopt a link bandwidth constraint $r_{ij} \le 1$ .  %\textcolor{green}{PL: Does this mean that $r_{ij}^d$ exist for all $d\in\mathcal{D}$ as long as there is an edge between $i$ and $j$?}  \nfc{Yes. In the case that routes are not pre-determined, $r_{ij}^d$ is a decision variable for all flows $d\in \D$.}


Each user $(i,d)\in \F$ is assigned a utility function $U_i^d$ of its rate $x_i^d$, which is % Each utility function $U_f$ is 
assumed to be upper-semicontinuous, proper, concave and non-decreasing. Indicative choices are $U_i^d(x) = w U(x)$ with $w\ge 0$ and $U$ is chosen as~\cite{srikant2013communication}: a) $U(x) = \log x$ (proportional fairness%\cite{kelly1998rate}
), b) $ U(x)= 
(1-\alpha)^{-1}x^{1-\alpha}, \ 0<\alpha<1$ (generalized fairness), %c) $U(x) = \sqrt{1-x^2}-1$, $x\le 1$  (used in Kuramoto oscillators), 
and many more. The goal of NUM is twofold: i) the users $(i,d)\in \F$ select the flow rates $\{x_i^d\}$ (congestion control), and ii) the nodes $i\in V$ select the link rates $\{r_{ij}^d\}$ (joint routing and MAC), so as to maximize the sum of user utilities subject to \emph{stability} and \emph{interference} constraints.

The NUM problem that we consider is given by:
	\begin{subequations}\label{eq:NUM}
	{\mathtight
		\begin{align}
		\underset{\{x^d_i\},\{r_{ij}^d\}}{\minimize} &\quad \sum_{i\in\mathcal{S}}\sum_{d\in \D_i} -U_i^d(x_i^d)\nonumber\\
		\stt 
		&\quad \sum_{j\in \Ne_i} r_{ji}^d + x^d_i \le \sum_{j\in \Ne_i} r_{ij}^d,\quad i\in\mathcal{S},\; d\in\mathcal{D}_i \label{eq:NUMa}\\
		& \sum_{j\in \Ne_i} r_{ji}^d  \le \sum_{j\in \Ne_i} r_{ij}^d, \quad i\in \mathcal{V},\; d\in \D_{-i}\label{eq:NUMaa}\\
		&\quad\sum_{d\in \D}\sum_{j\in \Ne_i} (r_{ij}^d + r_{ji}^d) \le 1,\quad i\in \mathcal{V}, \;d\in \D \label{eq:NUMb}\\
		&\quad r_{ij}^d \ge 0,\quad (i,j)\in \mathcal{E},\; d\in \D,\nonumber\\
		&\quad r^d_{ij}=0,\quad (i,j)\in \mathcal{E},\; i=d\in\D,\label{eq:NUMDummy}\\
		&\quad x^d_i \ge 0,\quad i\in \mathcal{S},\; d\in\D_i\nonumber
		\end{align}}
\end{subequations}
%
Notice that constraint~\eqref{eq:NUMDummy} captures that a user destination is a sink node with no outgoing traffic for that flow. 

\emph{Stability} refers to the requirement for bounded queues (\ie, bounded delays), and is defined separately for each destination $d$: for each node $i\in\mathcal{V}$ the cumulative incoming rate of traffic is less than or equal to the outgoing traffic. This is captured by the constraints~\eqref{eq:NUMa}, \eqref{eq:NUMaa}. 


\emph{Interference} captures conflict constraints in simultaneous transmissions over the same frequency band. %These are abstracted by $\mathbf{r}:=\{r_{ij}\} \in Co(\mathcal{R})$, the \emph{capacity region}, defined as the convex hull of discrete set $\mathcal{R}$ of $\{0,1\}^M-$vectors  representing the \emph{independent sets}, \ie, the subsets of links that can be simultaneously activated with no mutual interference. In the sequel, we consider a simplistic characterization of the interference constraints in cellular networks where: a node cannot simultaneously transmit to more than one and/or receive data from more than one transmitting node, whence $Co(\mathcal{R})$ is captured by:
%
%$$\sum_{j\in \Nout_i} r_{ij} + \sum_{j\in\Nin_i}r_{ji} \le 1,$$
We adopt here a simplistic interference model (see~\cite{srikant2013communication} for a more general model) 
in which a node \emph{cannot} simultaneously a) transmit data to more than one nodes, b) receive data from more than one nodes, and c) transmit and receive at the same time, cf.~\eqref{eq:NUMb}. %In summary, this introduces a \emph{concurrency constraint} of the form that the sum of total in-coming traffic plus the total outgoing traffic is bounded by 1:
%simultaneously a) transmit data to more than one nodes as well as b)receive data from more than one transmitting node, and 
%
%$$\sum_{j\in \Ne_i} r_{ij} + \sum_{j\in\Ne_i}r_{ji} \le 1,\quad \forall i\in V$$ 

%The NUM problem that we consider is given by:
%\begin{small}
%\begin{subequations}\label{eq:NUM}
%\begin{align}
%	\underset{\{x_f\},\{r_{ij}^d\}}{\minimize} & \underset{f\in F}{\sum} -U_f(x_f)\\
%	%\stt 
%	\text{s.t.}
%	&  \underset{j\in \Ne_i}{\sum} (r_{ji}^d - r_{ij}^d) + 
%	c_i^fx_f \le 0\label{eq:NUMa} & \forall i\in V, d\in \D\\
%	%&\underset{j\in \Ne_i}{\sum} (r_{ij} + r_{ji}) \le 1\label{eq:NUMb}\\
%	&\underset{d\in \D}{\sum}\underset{j\in \Ne_i}{\sum} (r_{ij}^d + r_{ji}^d) \le 1\label{eq:NUMb} & \forall i\in V\\
%	%& x_f \ge 0, r_{ij}^d \ge 0\label{eq:NUMc},
%	&r_{ij}^d \ge 0 & \forall (i,j)\in E, d\in \D\label{eq:NUMr}\\
%	& x_f \ge 0 & \forall f\in \F \label{eq:NUMf}
%\end{align}
%\end{subequations}
%\end{small}
%\begin{scriptsize}
%	\begin{subequations}\label{eq:NUM}
%			{\mathtight
%		\begin{align}
%		\underset{\{x^d_i\},\{r_{ij}^d\}}{\minimize} &\quad \sum_{i\in\mathcal{S}}\sum_{d\in \D_i} -U_i^d(x_i^d)\nonumber\\
%		\stt 
%		%\text{s.t.}
%		&\quad \sum_{j\in \Ne_i} r_{ji}^d + x^d_i \le \sum_{j\in \Ne_i} r_{ij}^d,\quad i\in\mathcal{S},\; d\in\mathcal{D}_i \label{eq:NUMa}\\
%		& \sum_{j\in \Ne_i} r_{ji}^d  \le \sum_{j\in \Ne_i} r_{ij}^d, \quad %i\notin\mathcal{S}\ \mathrm{ or }\ d\notin\mathcal{D}_i\cup\{i\}\label{eq:NUMaa}\\
%		%\nf{ (i\notin\mathcal{S} \ \& \ d\ne i) \quad  \mathrm{ or }  \quad (i\in\mathcal{S} \ \& \  d\notin\mathcal{D}_i})\nonumber\\
%		i\in \mathcal{V},\; d\in \D_{-i}\label{eq:NUMaa}
%		\\
%		%&\nf{\equiv (i\in S \ , \ d\notin\mathcal{D}_i\cup\{i\}) \quad \mathrm{ or } \quad (i\notin S \ , \ d \ne i)}\nonumber\\
%		%&\underset{j\in \Ne_i}{\sum} (r_{ij} + r_{ji}) \le 1\label{eq:NUMb}\\
%		&\quad\sum_{d\in \D}\sum_{j\in \Ne_i} (r_{ij}^d + r_{ji}^d) \le 1,\quad i\in \mathcal{V}, \;d\in \D \label{eq:NUMb}\\
%		%& x_f \ge 0, r_{ij}^d \ge 0\label{eq:NUMc},
%		&\quad r_{ij}^d \ge 0,\quad (i,j)\in \mathcal{E},\; d\in \D,\\%\setminus\{i\},\\
%		&\quad r^d_{ij}=0,\quad (i,j)\in \mathcal{E},\; i=d\in\D,\nonumber\\%\in\D\cap\{i\}\nonumber,\\
%		&\quad x^d_i \ge 0,\quad i\in \mathcal{S},\; d\in\D_i\nonumber
%		%&\quad \textrm{for all $d\in \D$},\nonumber
%		\end{align}}
%	\end{subequations}
%	\textcolor{green}{PL: Is there a reason that only certain constraints are numbered? }
%	\nfc{Not particularly, but it may make sense to ``group'' constraints, e.g., ~\eqref{eq:NUMa},\eqref{eq:NUMaa} are stability,~\eqref{eq:NUMb} is interference, and the rest are non-negativity. In passing, note also that our definition of `dummy' variables is not dummy at all, and is better than the NUM papers in the sense that we uniformly don't allow transmissions from a destination node. This is not explicitly stated in~\cite{lin2004joint,lin2006tutorial} although one can check that at optimality they are satisfied therein.}
%\end{scriptsize}
%
%
%\nfc{Note that $r^d_{ij}=0,\quad (i,j)\in \mathcal{E}, i=d\in\D$ is only needed to simplify notation in~\eqref{eq:NUMb} so that the two sums are indexed over all $d\in \D,j\in \Ne_i$ and combined into one. Such `dummy' variables are indeed `dummy,` in the sense that initializing $r^d_{ij}=0,\quad (i,j)\in \mathcal{E}, i=d\in\D,$ gives that $r^d_{ij} = \bar{r}^d_{ij}=0$ for all iterations, which is a nice general property of our algorithm.}
%
%the first constraint is for each $i\in V,d\in \D$,
%the second for each $i\in V$ and the last for each $f\in \F$, and $(i,j)\in E, d\in \D$, respectively.
The traditional cross-layer optimization%~\cite{tassiulas1992stability,lin2004joint,lin2006tutorial,
~\cite{srikant2013communication} amounts to solving the above minimization %\textcolor{green}{PL: shouldn't this involve all the constraints? or are they only considering~\eqref{eq:NUMa}-\eqref{eq:NUMb}?} \nfc{Only constraints~\eqref{eq:NUMa},~\eqref{eq:NUMaa} are relaxed in the Lagrangian, then dual function is computed and dual ascent is applied; cf.~\cite[pp. 6-8]{lin2004joint}} 
via dual decomposition, %where at each iteration: A) the dual function is computed, entailing two uncoupled sub-problems corresponding to i) congestion control and ii) joint scheduling/routing of transmissions 
which gives rise to the celebrated backpressure (or MaxWeight)  algorithm~\cite{srikant2013communication,tassiulas1992stability}. %) and B) dual ascent is used, which mimics the evolution of queue lengths, thus making the important connection between queues (user delays) and Lagrange multipliers (flow prices). It is important to highlight that computation of the dual function cannot, 
The algorithm has a natural intepretation of Lagrange multipliers as queue lengths. Nevertheless, in general (including the simplified interference model that we consider here), it requires solving a combinatorial problem at each iteration which is not amenable to distributed implementation. In contradistinction, our method is fully distributed and entails simple operations.% (at the cost of interpretability).
%since the MaxWeight algorithm is centralized (and may also be NP-hard under a general interference model).

%\nfc{Trim substantially and state final algorithm plus couple of supporting equations.}
We now show how to cast NUM into the setup of Problem~\eqref{prob:GenProblem}. For each node $i$, we define the primal vector $z_i$ to contain the incoming and outgoing link rates, as well as the exogenous flow rates (if some flows originate at node $i$). In essence, a link rate variable ``belongs'' to the node from which it originates. We introduce ``replicas,'', \ie, define $r_{ij,i}^d$ and $r_{ij,j}^d$, where the first variable ``belongs'' to node $i$ and the second is its estimate at node $j$. Therefore, the local decision vector for node $i\in\mathcal{V}$ is defined as
%$$x_i := [\{r_{ij,i}^d\}_{j\in\Ne_i,d\in \D},\{r_{ji,i}^d\}_{j\in\Ne_i,d\in \D}, \{x_f\}_{f:s_f=i}].$$
$$z_i := \left((r_{ij,i}^d,r_{ji,i}^d)_{j\in\mathcal{N}_i,d\in\D}, (x^d_i)_{d\in\D_i}\right),$$
%$$z_i := \left((r_{ij,i}^d)_{\substack{j\in\mathcal{N}_i\\ d\in \D_{- i}}},(r_{ji,i}^d)_{\substack{j\in\mathcal{N}_i\\ d\in\D_{- j}}}, (x^d_i)_{d\in\D_i}\right).$$
and its dimension is $n_i=|\mathcal{N}_i||\D|+|\D_i|$. Note that, throughout this section the variables are stacked by increasing order.
%\nfc{We should highlight the ordering of primal variables in $z_i$, so that they are consistent in the consensus constraint below.} \textcolor{green}{PL: We should emphasize that the $x_i^d$ variable above is there only if $i\in\mathcal{S}$.} \nfc{Yes, we have done that last sentence of left column in previous page.}

The edge-based consensus constraint~\eqref{eq:ds-2} is given by:
\begin{align*}
r_{ij,i}^d = r_{ij,j}^d,\quad r_{ji,i}^d = r_{ji,j}^d,\qquad d\in\D, (i,j)\in\mathcal{E}.
%r_{ji,i}^d &= r_{ji,j}^d,\qquad d\in\D, (i,j)\in\mathcal{E}.
\end{align*}
%\textcolor{green}{PL: Is it possible for a certain $d\in\mathcal{D}$ and $(i,j)\in\mathcal{E}$, to have both $r_{ij}^d\geq 0$ and $r_{ji}^d\geq 0$? Isn't the transmission for a certain destination one way?}\nfc{Good point. It is possible in the NUM formulation. In practice you don't want this (people have adopted variants of back-pressure where you only transmit across a link if this brings you closer to your destination; let's not go there).}
In terms of the notation defining the generic distributed optimization problem~\eqref{prob:GenProblem}, for $(i,j)\in\mathcal{E}$  one has $b_{(i,j)}=0$, and (assuming $i<j$ without loss of generality):
\begin{align*}
A_{ij}&: z_i\mapsto (r^d_{ij,i},-r^d_{ji,i})_{d\in\D},\\
A_{ji}&: z_j\mapsto (-r^d_{ij,j},r^d_{ji,j})_{d\in\D}. 
\end{align*}
   %\textcolor{green}{PL: Isn't the pair (i,j) unordered? In that case the definition of $A_{ij}$ above is self contradictory. We can change it to $A_{ij}: z_i\mapsto (r^d_{ij,i},-r^d_{ji,i})_{d\in\D}, (i,j)\in\mathcal{E}$ assuming an increasing ordering}\nfc{Yes; it's better as you recommend. In passing, note that the edge-constraint is general to capture such ``contradictory'' definitions.}
 
Utility functions are typically smooth, but may not have Lipschitz gradients so we set $f_i\equiv 0$, and proceed to define $g_i$\footnote{The negative utility is a scalar function and has therefore inexpensive proximal operator, which in several cases (e.g., logarithm) may be computed analytically.} to incorporate utilities and non-negativity constraints. The objective function for agent $i\in\mathcal{V}$ is given by:
$$g_i(z_i) =\sum_{d\in \D_i} -U_i^d(x_i^d)+ \delta_{Z_i}(z_i).$$
where 
\begin{align*}
Z_i=\{&\left((r_{ij,i}^d,r_{ji,i}^d)_{j\in\mathcal{N}_i,d\in\D}, (x^d_i)_{d\in\D_i}\right)\in\Re_+^{n_i},\\& \textrm{ and } r_{ij,i}^d=0, i=d\in\D\}.
\end{align*}
We define $h_i:\Re^{|\D\setminus\{i\}|+1}\to\Rinf$ to capture the constraints~\eqref{eq:NUMa}-\eqref{eq:NUMb}. Let $h_i = \delta_{C_i},$
with 
$$C_i =\left\{(v^{(1)},v^{(2)})\in\R^{|\D\setminus\{i\}|}\times\R\mid v^{(1)}\geq 0, v^{(2)}\leq 1\right\}.$$ 
Therefore, proximal mapping of $h_i$ is inexpensive. 

We proceed by defining $L_i \coloneqq (L_i^{(1)},L_i^{(2)})$. Let us first define the following notation:
	\begin{equation*}
	c_i^d(x)=\begin{cases}
	x & \quad d\in\D_i\\
	0 & \quad d\in\D_{-i}
	\end{cases}
	\end{equation*}
	If $i\in\mathcal{S}$ then
	\begin{align*}
	L_i^{(1)}: z_i &\mapsto  v_i^{(1)} =
	\Big(\sum_{j\in \Ne_i} (r_{ij,i}^d - r_{ji,i}^d)- c_i^d(x_i^d)\Big)_{ d\in\D \setminus \{i\}}.
	\end{align*}
	Otherwise, if $i\in\mathcal{V}\setminus\mathcal{S}$ then
	\begin{align*}
	L_i^{(1)}: z_i &\mapsto  v_i^{(1)} =
	\Big(\sum_{j\in \Ne_i} (r_{ij,i}^d - r_{ji,i}^d)\Big)_{ d\in\D \setminus \{i\}}.
	\end{align*}
	As for, $L_i^{(2)}$ we have %\footnote{Note that computations are repeated and can be re-used: $L_i^{(2)}z_i$ can be obtained by summing over $d\in\D$ the values $\sum_{j\in \Ne_i} r_{ij}^d, \sum_{j\in \Ne_i} r_{ji}^d$ computed by $L_i^{(1)}z_i$.}
	\begin{align*}
	%	L_i^{(1)}: z_i &\mapsto  v_i^{(1)} =\begin{cases}	\left(\sum_{j\in \Ne_i} (r_{ij,i}^d - r_{ji,i}^d)- x_i^d\right)_{ d\in\mathcal{D}_i}\\ %& \, i\in\mathcal{S},\;d\in\mathcal{D}_i\\	\left(\sum_{j\in \Ne_i} (r_{ij,i}^d - r_{ji,i}^d)\right)_{ d\notin\mathcal{D}_i\cup\{i\}}\\ %& \, i\in \mathcal{V}, d\notin\mathcal{D}_i\cup\{i\}	\end{cases}	 ,\\
	L_i^{(2)}: z_i &\mapsto  v_i^{(2)} = \sum_{d\in\D}\sum_{j\in \Ne_i} (r_{ij,i}^d + r_{ji,i}^d) \in \R.
	\end{align*}
	The transpose of $L_i$ is given by: 
	{\mathtight
	\begin{align*}
	L_i^\top\!:\! ((y_i^d)_{d\in\D\setminus\{i\} },y_i^{(2)}) &\mapsto  \big((u_{ij,i}^d,u_{ji,i}^d)_{j\in\mathcal{N}_i, d\in\D},(- y_i^d)_{d\in\D_i} \big)
	\end{align*}}
	where 
	$$u_{ij,i}^d = y_i^{(2)} + y_i^d,\; u_{ji,i}^d = y_i^{(2)} - y_i^d, \quad \forall d\in\D\setminus\{i\},$$
	and 
	$
	u_{ij,i}^d = u_{ji,i}^d = y_i^{(2)}$ if $i=d\in\mathcal{D}$. 

	It remains to write $\sum_{j\in\mathcal{N}_{i}}A_{ij}^{\top}{\bar{w}_{(i,j),i}}$ explicitly: %It can be evaluated as follows: 
	\begin{equation} \label{eq:-128}
	\sum_{j\in\mathcal{N}_{i}}A_{ij}^{\top}{\bar{w}_{(i,j),i}} =  \big((\bar{w}_{ij,i}^d,-\bar{w}_{ji,i}^d)_{j\in\mathcal{N}_i, d\in\D},(0)_{d\in\D_i} \big).
	\end{equation}
\Cref{Alg:NUM} summarizes the result of  applying 
\Cref{Alg:dist} to the NUM problem. For simplicity, all relaxation parameters $\lambda_i$ are set equal to $1$. 

Since for the NUM problem the smooth terms $f_i\equiv0$, in~\Cref{cond:cord}, the term $\|Q_i\|$  vanishes.
	%\begin{equation}\label{cond:NUM}\tau_i < \frac{1}{ \|\sigma_i L_i^\top L_i+\sum_{j\in\mathcal{N}_i}\kappa_{(i,j)}A_{ij}^\top A_{ij}\|}	\end{equation}
Furthermore, it is an easy exercise to check that $\|L_i^\top L_i\|=\|L_i L_i^\top\|=2|\mathcal{N}_i||\D|$. Given the definition of $A_{ij}$, a sufficient condition for convergence is to have 
\begin{equation}\label{eq:-13p}
\tau_i < \frac{1}{ 2\sigma_i|\mathcal{N}_i||\D| +\max_{j\in\mathcal{N}_i}\kappa_{(i,j)}}.
\end{equation}
\textcolor{blue}{The stepsizes are in the end not local because of $|\mathcal{D}|$.  Can we do anything for this?} 

In our simulations we consider small, medium, and large networks with $m=5,10,50$ nodes/agents, respectively. In all three cases we consider $5$ random flows. The communication graphs are generated randomly according to the Erd\H{o}s-Renyi model with parameter 0.05. We report the performance of \Cref{Alg:NUM} for three cases: $U(x)=\log(x)$, $U(x)=(1-\alpha)^{-1}x^{1-\alpha}$, with $\alpha=0.5$, and linear utility $U(x)=x$. 

For the stepsizes, we set $\kappa_{(i,j)}=2|\mathcal{D}|$ for all $(i,j)\in\mathcal{E}$, and $\sigma_i=2/|\mathcal{N}_i|$, $\tau_i=0.99/(6|\mathcal{D}|)$ (cf. \eqref{eq:-13p}). These values were selected empirically based on better performance of the algorithm, noting that in general larger stepsizes yield faster convergence. 

First, we consider the synchronous version of the algorithm. The performance of the algorithm is reported in \Cref{tab:table1} and \Cref{fig1}. The termination criteria is based on achieving a given relative error, $\|R^k\|/\|R^0\|$, where $R^k=\bar{v}^k-v^k$, and $v$ is the stacked primal and dual variables of all agents. It is observed that with all three utilities \Cref{Alg:NUM} achieves a moderate relative error fairly quickly, even for the large network. In fact, in most of the cases the residue is becoming three orders of magnitude smaller in less than $3000$ iterations. Furthermore, a higher accuracy is harder to achieve in the larger network, \Cref{fig1} (right). This is not unexpected, since \Cref{Alg:NUM} is a first order method. 

In \Cref{fig2} we compare the synchronous and asynchronous versions of the algorithm for the logarithmic utility function in the network with $m=10$. The x-axis denotes the total number of local updates (note that in the synchronous case at each iteration $m$ local updates are performed). For the asynchronous case, the activation probabilities of all the agents, $i=1,\ldots,m$, are set equal to $p_i=0.5$.  We observe that the algorithm takes roughly the same number of total local updates as the full version, \ie, even with random activation of agents the algorithm maintains its speed. This behavior is consistent and is observed for other utility functions and larger networks.  
 \iffalse 
\begin{table*}[h!t] % table for rand=0 
	\centering
	\caption{Total number of local iterations for different utility functions}
	\label{tab:table1}
	\begin{tabular}{c|ccc|ccc|ccc}
		\toprule 
		& \multicolumn{3}{c|}{Logarithmic} & \multicolumn{3}{c|}{Linear} & \multicolumn{3}{c}{Generalized fairness} \\
		$m$ & 1e-2 & 1e-3 & 1e-4 & 1e-2 & 1e-3 & 1e-4 & 1e-2 & 1e-3 & 1e-4\\
		\midrule 
		5 & 190  & 1090 & 2700 & 175 & 830 & 1980 & 1070 & 11940 & 60570 \\
		10 & 320 & 3980 & 16370 & 380 &  1820& 3540 &  1260
		& 33220& 255800 \\
		50 & 1500 & 9200 & 185750 & 1450 & 7750 & 43650 &  1500 & 63700 & 1209200 \\
	\end{tabular}
\end{table*} 
 
\begin{table*}[h!]  % the table for rand,1
	\centering
	\caption{Total number of local iterations for different utility functions \textcolor{red}{(old table)}}
	\label{tab:table1}
	\begin{tabular}{c|ccc|ccc|ccc}
		\toprule 
		& \multicolumn{3}{c|}{Logarithmic} & \multicolumn{3}{c|}{Linear} & \multicolumn{3}{c}{Generalized fairness} \\
		$m$ & 1e-2 & 1e-3 & 1e-4 & 1e-2 & 1e-3 & 1e-4 & 1e-2 & 1e-3 & 1e-4\\
		\midrule 
		5 & 500  & 2325 & 5165 & 265 & 1330 & 2415 &  4110 & 28240 & 75590 \\
		10 & 920 & 9860 & 33190 & 470 &  2130& 5220 &  3800
		& 109330& 468800 \\
		50 & 1600 & 13200 & 274650 & 1590 & 9500 & 47550 &  1650 & 116200 & 2147950 \\
	\end{tabular}
\end{table*} 

\begin{table*}[h!]  % the table for rand,2
	\centering
	\caption{Total number of local iterations for different utility functions \textcolor{red}{(rand=2, |flow|=5)}}
	\label{tab:table1}
	\begin{tabular}{c|ccc|ccc|ccc}
		\toprule 
		& \multicolumn{3}{c|}{Logarithmic} & \multicolumn{3}{c|}{Linear} & \multicolumn{3}{c}{Generalized fairness} \\
		$m$ & 1e-2 & 1e-3 & 1e-4 & 1e-2 & 1e-3 & 1e-4 & 1e-2 & 1e-3 & 1e-4\\
		\midrule 
		5 & 245  & 1070 & 2435 & 180 & 800 & 1550 & 1330
		& 3300 & 9990 \\
		10 & 290 & 1430 & 3430 & 350 & 1480 & 4540 &  1625 & 7365 & 22180  \\
		50 & 1400 & 12500 & 86150 & 1350 & 7750 & 45600 & 1650 & 59850 & 513600 \\
	\end{tabular}
\end{table*}
\fi
\iffalse % not per agent
\begin{table*}[h!]  % table for (rand=3, |flow|=5)
	\centering
	\caption{Total number of local iterations to reach $\|R^k\|/\|R^0\|<\epsilon_{tol}=10^{-2},10^{-3},10^{-4}$. }
	\label{tab:table1}
	\begin{tabular}{c|ccc|ccc|ccc}
		\toprule 
		& \multicolumn{3}{c|}{Logarithmic} & \multicolumn{3}{c|}{Linear} & \multicolumn{3}{c}{Generalized fairness} \\
		$m$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$\\
		\midrule 
		5 & 200  & 685 & 1145 & 140 & 725 & 1765 & 590
		& 6800 & 8740 \\
		10 & 450 & 3170 & 6630 & 360 & 1680 & 3500 & 1320 & 24910 & 78180  \\
		50 & 1450 & 16050 & 88800 & 1600 & 11800 & 79900 & 1550 & 106950 & 477550 \\
	\end{tabular}
\end{table*} 
\fi 

\begin{table*}  % table for (rand=3, |flow|=5)
	\renewcommand{\thetable}{\arabic{table}}
	\centering
	\caption{Number of iterations to reach $\|R^k\|/\|R^0\|<\epsilon_{tol}=10^{-2},10^{-3},10^{-4}$. }
	\label{tab:table1}
	\begin{tabular}{c|ccc|ccc|ccc}
		\toprule 
		& \multicolumn{3}{c|}{Logarithmic} & \multicolumn{3}{c|}{Linear} & \multicolumn{3}{c}{Generalized fairness} \\
		$m$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$\\
		\midrule 
		5 & 40  & 137 & 229 & 28 & 145 & 353 & 118
		& 1360 & 1748 \\
		10 & 45 & 317 & 663 & 36 & 168 & 350 & 132 & 2491 & 7818  \\
		50 & 290 & 3210 & 17760 & 320 & 2360 & 15980 & 310 & 21390 & 95510 \\
	\end{tabular}
\end{table*} 

\begin{figure*}
	\center
  \resizebox{0.9\linewidth}{!}{\input{TeX/Tikz/fig2}}
  \caption{The relative error for $m=10$ (left), and $m=50$ (right). %The $y$-axis denotes the order of reduction of the residue, $R^k=\bar{v}^k-v^k$, where $v$ is the stacked primal and dual variables of all agents. 
  }
  \label{fig1}
\end{figure*}

\begin{figure}
	\resizebox{0.9\linewidth}{!}{\input{TeX/Tikz/fig3}}
		\caption{The relative error for the logarithmic utility, synchronous and asynchronous schemes ($m=10$). }
		\label{fig2}
\end{figure}
 



   \iffalse 
\begin{table}[h!]
	\centering
	\caption{Logarithmic utility}
	\label{tab:table1}
	\begin{tabular}{c|ccc}
		\toprule
		m & 1e-3 & 1e-4 & 1e-5\\
		\midrule
		5 & 440 & 920& 1525\\
		10 & 1540 & 2900& 6080\\
		50 & 23500 & 54300 & 93100\\
		\bottomrule
	\end{tabular}
\end{table}
\iffalse 
\begin{table}[h!]
	\centering
	\caption{Piecewise-linear utility}
	\label{tab:table2}
	\begin{tabular}{c|ccc}
		\toprule
		m & 1e-3 & 1e-4 & 1e-5\\
		\midrule
		5 & 380 & 545& 715\\
		10 & 940
		 & 1110& 1360\\
		50 & 8400 & 9650 & 11350\\
		\bottomrule
	\end{tabular}
\end{table}\fi 

\begin{table}[h!]
	\centering
	\caption{Generalized fairness utility}
	\label{tab:table2}
	\begin{tabular}{c|ccc}
		\toprule
		m & 1e-3 & 1e-4 & 1e-5\\
		\midrule
		5 & 1855 & 2905& 4245\\
		10 & 5460
		& 10310& 15660\\
		50 & 147750 & * & *\\
		\bottomrule
	\end{tabular}
\end{table} \fi 
%\textcolor{green}{PL: The way \eqref{eq:NUMa} and \eqref{eq:NUMb} are defined are very confusing to me. For the same reason so is the definition of $L_i^{(1)}$ here. How about defining it like this: }
 %and $$u_i^d= - y_i^d,\quad   \forall d\in\D_i$$.Otherwise, if $i\in\mathcal{V}\setminus\mathcal{S}$ then\begin{align*}L_i^\top: ((y_i^d)_{d\in\D\setminus\{i\} },y_i^f) &\mapsto  \big((u_{ij,i}^d,u_{ji,i}^d)_{d\in\D\setminus\{i\}},(- y_i^d)_{d\in\D_i} \big),\end{align*}

%Finally, $h_i = \delta_{C_i},$ with $$C_i =\left\{(v^{(1)},v^{(2)})\in\R^{|\D|}\times\R\mid v^{(1)}\geq 0, v^{(2)}\leq 1\right\}.$$

%\nfc{What follows can be skipped and simply give the algorithm.}
%We proceed by defining the matrices as prescribed by our distributed optimization algorithm. First, define 
%$N = (N_{ij})$ and $b_{(i,j)}$
%for ${(i,j)\in E}$:
%$$N_{ij}x = (\{r^d_{ij,i}\}_d,\{-r^d_{ij,j}\}_d),\ \ \ 
%b_{(i,j)} = 0_{|\D|}.$$
%For each node $i$,
%order its neighbors $j\in \Ne_i$ (e.g., in ascending order), and consider $r_{ij,i}^d,r_{ji,i}^d$ for each neighbor, stacking the variables in blocks corresponding to a destination $d$. %, \ie, first block for flow $1$, second for flow $2$, etc  
%%The first operator $L_i^{(1)}$ is $|\D|$-dimensional. In matrix form, it can be
%The matrix $L_i^{(1)}$ is obtained by taking the Kronecker product of blocks ($1,-1$) repeated $|\Ne_i|$ times with the identity matrix $I_{|\D|}$,   
%%($N^T_i$ and $-N^T_i$) with $I_{|S|}$, 
%and appending with a matrix of dimension $|\D|\times s_i$
%of $-1$s and zeros for the $x_f$ variables. 
%Besides, $L_i^{(2)}$ is given by appending a an all-one row vector of length $2|\Ne_i||\D|$, with $s_i$ zeros.
%


%A distributed Newton method for NUM has been recently developed in~\cite{wei2013adistributed,wei2013bdistributed}, however it applies exclusively for wireline networks with predetermined routes. 

\begin{algorithm*}[ht!]
\caption{Synchronous \& asynchronous distributed primal-dual algorithm for NUM}
\label{Alg:NUM} 
\begin{algorithmic} 
		\algnotext{EndFor}
		\newcommand{\alignThm}[2][c]{%
			\setlength\myLength{\widthof{$z_{\mathcal{N}_i}^{k+1}$}}
			\ifstrequal{#1}{c}{
				\hspace*{0.5\myLength}
				\mathclap{#2}
				\hspace*{0.5\myLength}
			}{}
			\ifstrequal{#1}{l}{
				\mathrlap{#2}
				\hspace*{\myLength}
			}{}
			\ifstrequal{#1}{r}{
				\hspace*{\myLength}
				\mathllap{#2}
			}{}
		}%
	\item[]\textbf{Inputs:} %$\sigma_i,\tau_{i}>0$ for $i=1,\ldots,m$, and $\kappa_{(i,j)}>0$ for $(i,j)\in \mathcal{E}$. 
	{$z_i^0\in\R^{n_i}$, $y_i^0\in\R^{|\mathcal{D}\setminus\{i\}|+1}$, $w_{ij,i}^0,w_{ji,i}^0,r_{ij,i}^{d,0},r_{ji,i}^{d,0}\in\R$}.
%\vspace{-1.2em}
		\For{$k=0,1,\ldots$} 
		%		\item[]\textbf{for} $k=0,\ldots$ \textbf{do:} 
		\item[]  \fbox{
			\begin{minipage}[t][1.005\height]{0.35\textwidth-2\fboxsep-2\fboxrule\relax}
				\textbf{{I}: Synchronous version} 
				\vspace{10pt}
				
				\textbf{for} all agents $i=1,\ldots,m$ \textbf{do}
			\end{minipage} } \fbox {
			\begin{minipage}[t][1\height]{0.35\textwidth-2\fboxsep-2\fboxrule\relax}
				\textbf{ II: Asynchronous version} 
				
				\vspace{-1pt}draw r.v. $\epsilon_i^k$ according to $\mathbb{P}(\epsilon_i^0=1)=p_i$
				
				\vspace{-1pt}{\textbf{for} all agents $i$ with $\epsilon_i^k=1$ \textbf{do}} 
			\end{minipage} 
		}
		\vspace*{3pt}  
		\State {\bf Local updates}:
		\INDSTATE $\alignThm{\bar{w}_{ij,i}^{d,k}}=\tfrac{1}{2}\big(w_{ij,i}^{d,k}+w_{ij,j}^{d,k}\big)+\tfrac{\kappa_{(i,j)}}{2}\big(r_{ij,i}^{d,k}-r_{ij,j}^{d,k}\big)\ensuremath{,\quad\forall}j\in\mathcal{N}_{i},\forall d\in\mathcal{D}$
		\INDSTATE $\alignThm{\bar{w}_{ji,i}^{d,k}}=\tfrac{1}{2}\big(w_{ji,i}^{d,k}+w_{ji,j}^{d,k}\big)+\tfrac{\kappa_{(i,j)}}{2}\big(-r_{ji,i}^{d,k}+r_{ji,j}^{d,k}\big)\ensuremath{,\quad\forall}j\in\mathcal{N}_{i},\forall d\in\mathcal{D}$
		\INDSTATE  $\alignThm{\bar{y}_{i}^{k}}=y_{i}^{k}+\sigma_{i}L_{i}z_{i}^{k}-\sigma_{i}\mathcal{P}_{C_i}\big(\sigma_{i}^{-1}y_{i}^{k}+L_{i}z_{i}^{k}\big)$
		\INDSTATE $\alignThm{z_{i}^{k+1}}=\prox_{\tau_{i}g_{i}}\big(z_{i}^{k}-\tau_{i}L_{i}^{\top}\bar{y}_{i}^{k}-\tau_{i}\sum_{j\in\mathcal{N}_{i}}A_{ij}^{\top}{\bar{w}_{(i,j),i}^{k}}\big)$ where the last term is given by \eqref{eq:-128}.  
		\INDSTATE $\alignThm{y_{i}^{k+1}}=\bar{y}_{i}^{k}+\sigma_{i}L_{i}(z_{i}^{k+1}-z_{i}^{k})$
		\INDSTATE $\alignThm{w_{ij,i}^{d,k+1}}=\bar{w}_{ij,i}^{d,k}+\kappa_{(i,j)}(r_{ij,i}^{d,k+1}-r_{ij,i}^{d,k})\quad\forall j\in\mathcal{N}_{i},\forall d\in\mathcal{D}$
		\INDSTATE $\alignThm{w_{ji,i}^{d,k+1}}=\bar{w}_{ji,i}^{d,k}-\kappa_{(i,j)}(r_{ji,i}^{d,k+1}-r_{ji,i}^{d,k})\quad\forall j\in\mathcal{N}_{i},\forall d\in\mathcal{D}$
		%\INDSTATE $w_{ji,i}^{k+1}=\bar{w}_{ji,i}^{k}+\kappa_{(i,j)}(z_{ii}^{k+1}-z_{ii}^{k}),\textrm{ for all }j\in\mathcal{N}_{i}^{\textrm{out}}$
		\State {\bf Broadcast of information}:
		\INDSTATE Send $r_{ij,i}^{d,k+1}$, $r_{ji,i}^{d,k+1}$,  $w_{ij,i}^{d,k+1}$, and $w_{ji,i}^{d,k+1}$ to agent $j$ for all $j\in\mathcal{N}_i$, $d\in\mathcal{D}$ 
		\EndFor
\end{algorithmic}
\end{algorithm*}




==> TeX/Text/Proofs/proofitemize.tex <==
\package{clevethm} provides a {\tt proofitemize} list for the layout of proofs of theorems which are split into a list of statements (cf. \Cref{sec:Enumerate}).

\noindent
\begin{minipage}[t]{.6\linewidth}%
	\vspace*{-5pt}%
\begin{lstlisting}
\begin{thm}
The following hold
\begin{enumerate}
	\item\label{1st}$1=1$
	\item\label{2nd}$1\leq2$
\end{enumerate}
\begin{proof}
\begin{@({\color{red}proofitemize})@}
	\item\ref{1st}. The proof is based on the twice-epidifferentiability of $x\mapsto 1$.
	\item\ref{2nd}. Too difficult.\qedhere
\end{@({\color{red}proofitemize})@}
\end{proof}
\end{thm}
\end{lstlisting}
\end{minipage}%
\hfill%
\begin{minipage}[t]{.39\linewidth}%
	\vspace*{0pt}%
	\standalone{proofenumerate}%
\end{minipage}



==> TeX/Text/Vu_Condat__Puya_Latafat_s_conflicted_copy_2018-05-23_.tex <==
%!TEX root = ../../paper.tex
\hl{
Recently, the design of primal-dual algorithms for solving  problem~\eqref{eq:equiv-probt} (as well as special cases for $f\equiv 0$ or $g\equiv0$) has received a lot of attention in the literature.  
% The popularity of this class of algorithms is due to the fact that they involve the proximal mappings of $g$ and $h$, the gradient of $f$ and the linear mapping $L$ and its adjoint are evaluated separately without the need to invert matrices or to solve inner loops. 
%The convergence analysis techniques for primal-dual algorithms in the literature are varied. 
Most of the existing approaches can be interpreted as  applications of one of the three main splittings techniques: Forward-Backward (FB), Douglas-Rachford (DR), and Forward-Backward-Forward (FBF) splittings \nf{reference for each splitting technique; preferably one book, e.g. Rockafellar} \cite{vu2013splitting,condat2013primal,briceno2011monotone+,combettes2012primal}, while others employ different tools \nf{explain} to establish convergence  \cite{chambolle2011first,drori2015simple}.}  

% Furthermore, notice that we have generalized and simplified the analysis in \cite[Sec. 5]{Latafat2017} for primal-dual algorithms by considering stepsize matrices in place of scalars, 
% In fact, the proposed algorithm is the result of solving the primal-dual optimality conditions for~\eqref{eq:equiv-prob} using a new three term splitting: \emph{Asymmetric Forward-Backward Adjoint} (AFBA), proposed recently by the authors~\cite[Alg. 1]{Latafat2017}. The operator defining this splitting involves an asymmetric preconditioning that gives it great flexibility and is the key to unifying primal-dual proximal algorithms.

\hl{
In our previous work \cite{Latafat2017}, we proposed a new three-term splitting method, called \emph{Asymmetric Forward-Backward Adjoint} (AFBA), and established a unifying framework for analyzing primal-dual algorithms as fixed point iterations.  %This splitting uses an operator of the form defined in~\eqref{eq:op2} and involves an additional dynamic stepsize. 
In specific, it was shown in \cite[Sec. 5]{Latafat2017} that several primal-dual algorithms such as  \cite{combettes2012primal,briceno2011monotone+,chambolle2011first,vu2013splitting,condat2013primal,drori2015simple} %as well as other new primal-dual algorithms 
can be cast as fixed-point iterations of the operator $T$, as  defined in~\eqref{eq:op2}, for a particular selection of matrices $S$, $P$, $K$. Additionally, the convergence analysis can be carried out via a Fej\'er-type inequality of the form \Cref{thm:synch} (for specially selected $\tilde{P}$ and $S$). 
} %Consequently, a wide array of primal-dual algorithms may be analyzed in a unified fashion.  We refer the reader to \cite[Sec. 5, Fig. 1]{Latafat2017} for a detailed discussion on the relation between primal-dual algorithms. }
%
% It was shown in  \cite[Sec. 5]{Latafat2017} that based on the new splitting  that many of the existing primal-dual algorithms including \cite{combettes2012primal,briceno2011monotone+,chambolle2011first,vu2013splitting,condat2013primal,drori2015simple} as well as other new primal-dual algorithms can be cast as fixed point iterations of the operator $T$ defined in~\eqref{eq:op2} for different matrices $S$, $P$, $K$. Consequently, a wide array of primal-dual algorithms may be analyzed in a unified fashion. The general primal-dual framework of \cite[Alg. 3]{Latafat2017} involves an additional dynamic stepsize. While the dynamic stepsize may improve the performance, it is disadvantageous in distributed optimization in large-scale systems where global coordination may be infeasible. For this reason in \eqref{eq:op2} we do not include any dynamic stepsize. 
 % Notice that \Cref{Alg:synch-1} (with $\Sigma=\sigma\I$, $\Gamma=\gamma\I$) may be seen as \cite[Alg. 3]{Latafat2017} applied to the dual problem with $\theta=1$, $\mu=1$ (in that work), and when the smooth term is zero. %It is also related to the algorithm of \cite{drori2015simple} that considers problem~\eqref{eq:equiv-probt} without the nonsmooth function $g$, \ie, $g\equiv0$. 
 % We refer the reader to \cite[Sec. 5, Fig. 1]{Latafat2017} for a more detailed relation between primal-dual algorithms. 
 
\hl{
%Capitalizing on this unifying framework, 
%
In this paper, an key contribution is the development of a new primal-dual operator splitting algorithm with \emph{diagonal} matrix $S$ in \Cref{Alg:synch-1}, which is integral for developing a \emph{fist of its kind} block-coordinate algorithm (cf. \Cref{subsec:CD}), that is further capitalized on for devising new randomized distributed algorithms for multi-agent optimization (cf. \Cref{sec:DistOpt}). 
}

\hl{
In order to establish a connection with the current state-of-the-art, we revisit the celebrated algorithm of V\~u and Condat \cite{condat2013primal,vu2013splitting} under the prism of fixed-point iterations with the operator $T$ in \eqref{eq:op2}, for a special selection of matrices $S$, $P$, $K$. }
%
% Among the existing primal-dual algorithms, the one of  V\~u and Condat \cite{condat2013primal,vu2013splitting} can be used to solve problem~\eqref{eq:equiv-probt}
% It may be shown that all the aforementioned algorithms  by showing Fej\'er monotonicity of the generated sequence is the space equipped with $\langle\cdot,\cdot\rangle_S$ where $S$ is different depending on the algorithm. A popular primal-dual algorithm is the one of V\~u and Condat. To demonstrate and compare in what follows we explicitly derive the algorithm using the operator $T$ in \eqref{eq:op2} with different $S$, $P$, $K$.  
%  Our goal here is to demonstrate that, unlike \Cref{Alg:synch-1}, for other closely related primal-dual algorithms such as the V\~u-Condat algorithm the Fej\'er monotonicity of the generated sequence holds in the space equipped with $\langle\cdot,\cdot\rangle_S$ where $S$ is not diagonal. In what follows we briefly describe the matrices $S$, $P$, $K$ for the algorithm of V\~u and Condat \cite{condat2013primal,vu2013splitting}. We note that this analysis leads to 
% less restrictive stepsizes conditions. 
 % 
  In \cite{condat2013primal} Condat considers  problem~\eqref{eq:equiv-probt}, while V\~u \cite{vu2013splitting} considers the following variant: 
 \begin{equation} \label{prob:gen}
   \underset{x\in\R^n}{\minimize}\ {f}({x})+{g}({x})+(h\oblong l)({L}{x}),
      \end{equation}
%\ie, the nonsmooth term $h$ is replaced by $h\oblong l$, 
where $l$ is a strongly convex  function and $\oblong$ represents the infimal convolution~\cite{bauschke2011convex}.  %\ie the problem becomes: \nf{better to write the formula for infimal convolution explicitly}.   
%   
%Here we include $l$ in the problem for the sake of comparison.
%
For this problem, %in addition to \Cref{ass:1}, we assume that
an additional assumption is that the conjugate of $l$ is continuously differentiable, $\nabla l^*$ is $\beta_l$-Lipschitz continuous with respect to a metric $G\succ0$, for some $\beta_l\ge 0$, cf. \eqref{eq:Lip}. 
We note in passing, that it is possible to derive a variant of \Cref{Alg:synch-1} for this problem, however, we do not pursue this in the sequel and focus explicitly on problem~\eqref{eq:equiv-probt} (which is a special case of~\eqref{prob:gen}  %additionally 
for $l=\delta_{\{0\}}$ %, the infimal convolution $h\oblong l=h$, $l^*\equiv0$ and 
whence the algorithm~\cite[Sec. 4]{vu2013splitting} reduces to \cite[Alg. 3.2]{condat2013primal}) 
for clarity of exposition and length considerations, in what follows. 

One can verify that the V\~u-Condat algorithm is a special case of the fixed point iterations~\eqref{eq:op2},~\eqref{eq:op1} for % with $H=P+K$ and $S$ defined as follows: 
\begin{equation}\label{S:vu-condat}
S=\begin{pmatrix}
\Sigma^{-1} & {L}\\
{L}^\top & \Gamma^{-1}
\end{pmatrix},
	\end{equation}
	 \begin{equation*} %\label{eq:PD-Vu}
	 P=\begin{pmatrix}
	 \Sigma^{-1} & {L}\\
	 {L}^\top & \Gamma^{-1}
	 \end{pmatrix}, \quad 
	 K=\begin{pmatrix}
	 0 & -{L}\\
	 {L}^\top & 0
	 \end{pmatrix}.
	 \end{equation*} 
Observe the non-diagonal structure of $S$ for the V\~u-Condat algorithm in contrast to our diagonal selection %(contrast~\eqref{S:blkdiag} and 
\eqref{S:vu-condat}. 
%
It is easy to check that the selection of $S$, $P$, $K$ in \eqref{S:vu-condat} yields $S^{-1}(H+M^\top)=I$, whence in proximal form, the operator defined in~\eqref{eq:op2},~\eqref{eq:op1} becomes:
	\begin{subequations} \label{eq:T-Vu}
		\begin{align}
		\bar{u} & =\prox_{h^{*}}^{\Sigma^{-1}}(u-\Sigma\nabla l^*(u)+\Sigma L{x})\\
		\bar{x} & =\prox_{g}^{\Gamma^{-1}}(x-\Gamma\nabla f(x)-\Gamma L^{\top}(2\bar{u}-u))\\
		Tz & =(\bar{u},\bar{x}).
		\end{align}
	\end{subequations} 
	%The analysis \nf{follows the same lines as} in \Cref{subsec:NewPD}. %and uses the operator $T$ as in\nf{~\eqref{eq:op2},~\eqref{eq:op1}} but with 
	% The algorithm is then defined as iterative applications of $T$ as in \eqref{eq:fixedpointT}.
For the sake of comparison with \cite{condat2013primal,vu2013splitting}, in this subsection we consider the relaxed iteration $z^{k+1}=z^k+\lambda (Tz^k-z^k)$ for some $\lambda\in(0,2)$ (which we opted to exclude from the analysis of our proposed method solely for the purpose of simplicity). When $\Sigma$ and $\Gamma$ are replaced with scalars $\sigma,\gamma$, the algorithm of \cite{vu2013splitting,condat2013primal} is precisely recovered.  % similarly,   %additionally 
%when $l=\delta_{\{0\}}$ %, the infimal convolution $h\oblong l=h$, $l^*\equiv0$ and 
%problem~\eqref{prob:gen} the algorithm reduces to \cite[Alg. 3.2]{condat2013primal} (where in both cases a fixed relaxation parameter $\lambda$ is used).  
	% In \cite{condat2013primal,vu2013splitting} relaxed iterates are considered. Here we have avoided this for simplicity. 

In order to establish convergence of this scheme, \Cref{ass:2} is replaced with the following condition: 
\hide{
	\begin{subequations}\label{eq:Vu-Condat}
	 		\begin{align}
			&\Sigma^{-1}-\tfrac{\beta_l}{2(2-\lambda)}G\succ0,\\
	 		&\Gamma^{-1}-\tfrac{\beta_f}{2(2-\lambda)}Q-L^{\top}\left(\Sigma^{-1}-\tfrac{\beta_l}{2(2-\lambda)}G\right)^{-1}L\succ0.
	 		\end{align}
	\end{subequations}
	  Notice that if $l=\delta_{\{0\}}$, then $l^*\equiv0$ and $\beta_l=0$. Problem \eqref{prob:gen} simplifies to~\eqref{eq:equiv-probt}, and the  condition~\eqref{eq:Vu-Condat} reduces to}
   \begin{equation}\label{eq:Vu-Condat}
   \Gamma^{-1}-\tfrac{\beta_f}{2(2-\lambda)}Q-L^{\top}\Sigma L\succ0.
   \end{equation} 
   \nf{I deleted here the general condition for $\ell \ne \delta_{\{0\}}$, for simplicity.} 
   \textcolor{orange}{I think it is better to keep it because we use it below in equation (27) for comparison. }
		% \begin{equation} \label{eq:Vu-Condat}
	 % 		 \Sigma^{-1}\succ\tfrac{\beta_l}{2}G, \; \; \Gamma^{-1}-\tfrac{\beta_f}{2}Q-L^{\top}\left(\Sigma^{-1}-\tfrac{\beta_l}{2}G\right)^{-1}L\succ0.
	 % 	\end{equation}
	Under this condition, the convergence of the algorithm is established by arguing similarly as in  \Cref{thm:synch}, where the Fej\'er-type inequality becomes:
  \begin{equation}
    \|z^{k+1}-z^\star\|_{S}^2 {}\leq{}\|z^k-z^\star\|_{S}^2 -  \lambda\|z^{k+1}-z^k\|_{2{\hat{P}}-\lambda S}^2,\label{Fej:synch3}
    \end{equation}
	  with $S$ defined in \eqref{S:vu-condat} and $\hat{P}$ given by:
		\begin{equation*} %\label{eq:tildeP-Vu}
 		\hat{P}\coloneqq\begin{pmatrix}
 		\Sigma^{-1}-\tfrac{\beta_l}{4}G & {L} \\
 		{L}^\top & \Gamma^{-1}-\tfrac{\beta_f}{4}Q 
 		\end{pmatrix}.
 		\end{equation*}

% The convergence analysis in this case is similar to that of \Cref{Alg:synch-1} but with $S$ as in \eqref{S:vu-condat} and $\tilde{P}$ in \eqref{eq:main-innerprod} replaced with
% 		\begin{equation*} %\label{eq:tildeP-Vu}
%  		\hat{P}\coloneqq\begin{pmatrix}
%  		\Sigma^{-1}-\tfrac{\beta_l}{4}G & {L} \\
%  		{L}^\top & \Gamma^{-1}-\tfrac{\beta_f}{4}Q 
%  		\end{pmatrix}.
%  		\end{equation*}
% Therefore, 
This analysis \emph{generalizes} the result in \cite[Thm. 3.1]{condat2013primal}, \cite[Cor. 4.2]{vu2013splitting} and \cite[Prop. 5.1]{Latafat2017} where the Lipschitz continuity is with respect to the canonical norm and the stepsizes are assumed to be scalar. 

\hl{
   Our main goal here was to demonstrate the non-diagonal structure of $S$ for the V\~u-Condat algorithm. In the rest of this section we briefly point out that our analysis leads to less conservative conditions as compared to \cite{vu2013splitting,condat2013primal,combettes2014forward}. 
   Notice that the proof technique used in the aforementioned papers is based on showing that the algorithm can be written as a forward-backward iterations. Therefore the stepsize condition ensures that the operator is averaged. While the condition in \eqref{eq:Vu-Condat} only ensures that the Fej\'er-type inequality \eqref{Fej:synch3} holds, which is sufficient for convergence (refer to \cite[Rem. 3.1]{Latafat2017} for more details regarding the properties of operator $T$ defined in \eqref{eq:op2} in general). Consequently, even in the scalar case condition \eqref{eq:Vu-Condat} allows larger stepsizes compared to \cite{vu2013splitting,condat2013primal} (see \cite[Rem. 5.6]{Latafat2017}).}

   % We emphasize that \cite[Thm. 3.1]{condat2013primal} uses a different proof technique and shows that the algorithm can be written as a forward-backward iterations. 
   %Modifying the proof of  \cite[Thm. 3.1]{condat2013primal} to account for the metric of Lipschitz continuity and stepsize matrices leads to \emph{more conservative} conditions. %This is true even in the scalar case when relaxation parameter (see \cite[Rem. 5.6]{Latafat2017}).
    % Notice that \cite[Thm. 3.1]{condat2013primal} uses a different proof technique by showing that the algorithm can be written as a forward-backward iterations. 
    % This leads to more conservative stepsize condition in presence of relaxation parameter.
   % 
	% In \cite{vu2013splitting,condat2013primal}, the metrics $Q$ and $G$ are the identity.

	 In \cite{combettes2014forward,pesquet2014class} the authors propose a variable metric version of the algorithm with a preconditioning that accounts for the general Lipschitz metric. This is done by setting the stepsizes to be proportional to the inverse of the Lipschitz metrics. 
		In comparison, our approach yields a wider range of parameters, where the stepsizes are not limited to be proportional to the inverse of the Lipschitz metric, and can take {larger} values thus achieving generally faster convergence. In order to compare let us set $\Gamma=\mu Q^{-1}$ and $\Sigma= \nu G^{-1}$ for some $\mu,\nu>0$. 
		For simplicity and without loss of generality let $\beta_l=1$, $\beta_f=1$.  With such a special choice of $\Sigma$ and $\Gamma$, \eqref{eq:Vu-Condat} simplifies to 
   \begin{equation}
   (\mu^{-1}-\tfrac{1}{2(2-\lambda)})(\nu^{-1}-\tfrac{1}{2(2-\lambda)})Q-L^{\top}G^{-1}L\succ0,  \label{eq:ourVu}
   \end{equation}
   whereas the condition required in \cite{combettes2014forward,pesquet2014class} is $\lambda\in(0,1]$ and  
   \begin{equation}\label{eq:theirVu}
   \mathtight{\frac{\delta}{1+\delta}>\frac{\max\{\mu,\nu\}}{2}\; \textrm{with } \; \delta=\tfrac{1}{\sqrt{\nu\mu}}\|G^{-1/2}LQ^{-1/2}\|^{-1}-1.}
   \end{equation}
   It is not hard to check that condition,~\eqref{eq:ourVu}, is always less restrictive than~\eqref{eq:theirVu}. As an example, let $G^{-1/2}LQ^{-1/2}=I$  and set $\mu=1.5$, then \eqref{eq:ourVu} simplifies to $\nu<\tfrac{1}{6.5}$ whereas \eqref{eq:theirVu} becomes $\nu<\tfrac{1}{24}$. 
   
  
    \done
